Including Everyone, Everywhere: Understanding Opportunities and Challenges of Geographic Gender-Inclusion in OSS

The gender gap is a significant concern facing the software industry as the development becomes more geographically distributed. Widely shared reports indicate that gender differences may be specific to each region. However, how complete can these reports be with little to no research reflective of the Open Source Software (OSS) process and communities software is now commonly developed in? Our study presents a multi-region geographical analysis of gender inclusion on GitHub. This mixed-methods approach includes quantitatively investigating differences in gender inclusion in projects across geographic regions and investigate these trends over time using data from contributions to 21,456 project repositories. We also qualitatively understand the unique experiences of developers contributing to these projects through a survey that is strategically targeted to developers in various regions worldwide. Our findings indicate that gender diversity is low across all parts of the world, with no substantial difference across regions. However, there has been statistically significant improvement in diversity worldwide since 2014, with certain regions such as Africa improving at faster pace. We also find that most motivations and barriers to contributions (e.g., lack of resources to contribute and poor working environment) were shared across regions, however, some insightful differences, such as how to make projects more inclusive, did arise. From these findings, we derive and present implications for tools that can foster inclusion in open source software communities and empower contributions from everyone, everywhere.

==> RW.tex <==
\begin{itemize}
    \item Understanding how developers contribute to Open Source~\cite{zlotnick2017github}
    \item what are the drop out rates to why people contribute~\cite{miller2019people}
    \item GitHub State of the Octoverse Survey 2018\cite{github2018octoverse} and 2019\cite{github2019octoverse}
\end{itemize}

\subsection{Barriers To Participation}
\begin{itemize}
    \item Barriers and Motivations for One Time Contributors to Open Source~\cite{lee2017understanding}
    \item Barriers for women to contributing to Stack Overflow~\cite{ford2016paradise}
    \item gender hiding not a viable decision for women~\cite{vedres2019gendered}
    \item gender bias is largely challenging to detect on GitHub~\cite{imtiaz2019investigating}
    
\end{itemize}

\subsection{Global Software Development}
DIversity in 
\begin{itemize}
    \item Higher acceptance rates were observed for all but one country when pull requests were evaluated by developers from the same country~\cite{rastogi2018relationship}
    \item women only communities~\cite{singh2019women}
\end{itemize}

